Behavior Alignment via Reward Function Optimization

Designing reward functions for efficiently guiding reinforcement learning (RL) agents toward specific behaviors is a complex task. This is challenging since it requires the identification of reward structures that are not sparse and that avoid inadvertently inducing undesirable behaviors. Naively modifying the reward structure to offer denser and more frequent feedback can lead to unintended outcomes and promote behaviors that are not aligned with the designer's intended goal. Although potential-based reward shaping is often suggested as a remedy, we systematically investigate settings where deploying it often significantly impairs performance. To address these issues, we introduce a new framework that uses a bi-level objective to learn \emph{behavior alignment reward functions}. These functions integrate auxiliary rewards reflecting a designer's heuristics and domain knowledge with the environment's primary rewards. Our approach automatically determines the most effective way to blend these types of feedback, thereby enhancing robustness against heuristic reward misspecification. Remarkably, it can also adapt an agent's policy optimization process to mitigate suboptimalities resulting from limitations and biases inherent in the underlying RL algorithms. We evaluate our method's efficacy on a diverse set of tasks, from small-scale experiments to high-dimensional control challenges. We investigate heuristic auxiliary rewards of varying quality -- some of which are beneficial and others detrimental to the learning process. Our results show that our framework offers a robust and principled way to integrate designer-specified heuristics. It not only addresses key shortcomings of existing approaches but also consistently leads to high-performing solutions, even when given misaligned or poorly-specified auxiliary reward functions.

==> Notes/header.tex <==
% Get better typography
% \usepackage[protrusion=true,expansion=true]{microtype}		

% Small margins
%\usepackage[top=2cm, bottom=2cm, left = 1cm, right = 1cm,columnsep=2

% For basic math, align, fonts, etc.
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{bbm}
\usepackage{mathtools}
\usepackage{mathrsfs}
\mathtoolsset{showonlyrefs}

\newtheorem{defn}{Definition}[]
\newtheorem{thm}{Theorem}[]
\newtheorem{claim}{Claim}[]
\newtheorem{lemma}{Lemma}[]
\newtheorem{prop}{Property}[]
\newtheorem{ass}{Assumption}[]
\newtheorem{cor}{Corollary}[]

% For creating sub-groups of Assumptions/Theorems etc.
\newtheorem{assumpA}{Assumption}
\renewcommand\theassumpA{A\arabic{assumpA}}

\usepackage{courier} % For \texttt{foo} to put foo in Courier (for code / variables)

\usepackage{lipsum} % For dummy text

% For images
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage[space]{grffile} % For spaces in image names

% For bibliography
\usepackage[round]{natbib}

% For links (e.g., clicking a reference takes you to the phy)
\usepackage{hyperref}

\usepackage{theoremref}
% For color
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{xcolor}
\definecolor{dark-red}{rgb}{0.4,0.15,0.15}
\definecolor{dark-blue}{rgb}{0,0,0.7}
\hypersetup{
    colorlinks, linkcolor={dark-blue},
    citecolor={dark-blue}, urlcolor={dark-blue}
}


% Macros
\newcommand{\yash}[1]{\textcolor{blue}{[#1---yash]}}
\newcommand{\todo}[1]{\textcolor{red}{[TODO: #1]}}


\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}


\usepackage{algpseudocode}
% \usepackage[noend,linesnumbered,ruled]{algorithm2e}
\usepackage[vlined,linesnumbered,ruled,algo2e]{algorithm2e}
% \usepackage[algo2e]{algorithm2e} 
\SetKwProg{Fn}{Function}{}{}
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line

% Miscelaneous headers
\usepackage{multicol}
\usepackage{enumitem}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{nicefrac}       % compact symbols for 1/2, etc.


==> oldintro.tex <==
%
The success of any reinforcement learning (RL) algorithm hinges on the availability of a useful reward function. 
%
%
% Unfortuna0tely, it is often non-trivial to design a reward function for a new problem that allows an agent to quickly converge to the desired behavior.
%
However, several studies have highlighted that humans are not good at % intuition may not be well adept at 
designing reward functions that cause  RL agents to learn desired behaviors quickly; % an agent to quickly learn desired behaviors; 
and ill-specified rewards might result in sub-optimal and undesired agent behavior \citep{ho2015teaching,ho2019people}. The spectrum of reward functions design starts from sparse rewards, where the agent receives a positive value for reaching a goal state\footnote{Sparse rewards just don't mean receiving a zero value at every other state, more generally it means not getting informative/discriminative reward between different actions at a given state, for example receiving a -1 rewards at each step is also not dense (is still sparse), as it doesn't help the agent discern between the effect of different actions available at the given state}, 
to dense rewards which evaluate an agent's actions at each step. There also exists various intermediate reward functions too which might  reward the agent  exhibiting partially correct behavior for e.g., often agents receive positive rewards for reaching sub-goal (/bottleneck) states which are potentially believed to be important to solve the task. 

Figuring out if a given reward function will induce the desired behavior is often as difficult as solving the problem, and hence it is not possible to tell beforehand whether a given reward function induces the right behavior unless we rely on human intuition for which we can't say for sure is most often correct or not. The reward functions for which we can intuitively answer the above questions often tend to be sparse, as it is easier to encode desired behavior often as reaching a goal state. Yet, using these sparse rewards signal can make the optimization process painfully slow -- particularly because the agent has to rely on extensive exploration to have a possibility of encountering some positive reward.  

In contrast, as designers, we often have access to a lot more information about the problem that we can potentially encode in a sparse reward function, and adding that information into the reward naively starts blurring the picture about the correct behavior-inducing capability of this new information-rich reward functions (which is also denser) based on human intuition, as the agent starts to become more and more susceptible to reward hacking \cite{}. Methods like potential-based reward shaping \cite{ng1999policy} have been designed such that information like the above may be incorporated with a sparser reward signal to potentially accelerate learning. 

Hence, the setting we consider in this paper is one where, the primary reward is specified by the environment, which encodes the desired behavior that 

% 
 % \dg{Is this a complete sentence, it does not seem like a complete thought. You might instead state this as an assumption, e.g., It can be easy to provide the agent with a single reward that induces the desired behavior, but the sparsity of this reward signal makes optimization slow.}
 % However, specifying a reward function that evaluates the agent's achievement of desired behavior at the end of trying to solve the task, may seem relatively easy. Yet, optimizing the sparse rewards for learning can be exceedingly difficult due to the extensive need for exploration and lack of immediate evaluative feedback \citep{hare2019dealing}. 
 % to the substantial exploration required and the limited instructive feedback available \citep{hare2019dealing}.

%
% However, it might be relatively easy to specify a reward function that provides evaluation at the end when the agent achieves the desired behavior, but it might not be directly useful as it can be prohibitively hard to optimize for such sparse rewards \citep{hare2019dealing}.
% Meaning : n this sentence I am trying to say that often it is easy to define sparse rewards for the agent where the agent learns if the strategy it followed to solve a given task lead the desired end goal or not. Although speciyfing this sparse reward is easy based on definingi it on the end goal state/outcome, using this reward to learn a pol;icuy can take learning prohibitely long as reaching the goal states might take a lot of exploration and very less instructive feedback
%
% % \dg{I did not see this sentence coming. Maybe set these sentences (previous and this one) up as a spectrum of reward functions with different trade-offs then introduce them.}
% In contrast, using rewards that provide immediate feedback %frequent evaluations 
% might accelerate  the agent's learning, but  are often non-trivial to design. %it is non-trivial to design 
% As most of the rewards that are defined for immediate feedback leverage 
% % \dg{This is a huge point that goes beyond this paper, but is maybe the best framing for it. Based on a human intuition does a reward function lead to the desired behavior. The answer is most the time we don't know. The reward functions we can answer this for are often sparse... Our approach assumes that the agent is given a primary reward function that will induce desired behavior and given access to prior knowledge in the form of axuliary rewards. Instead of the human having to say how these axuliarly tasks are relevant it is part of the agent's part job to identify if any of these axualiary rewards are useful for maximizing the primary reward function.} 
% heuristics based on human intuition and it is unclear how to ascertain if such dense rewards would also induce the desired behavior.
% %
% Consequently,  either various \textit{auxiliary rewards} are used in practice that might result in sub-optimal behavior \citep{openai}, or potential-based reward shaping \citep{ng1999policy} is used that can have its own limitations, as we discuss later.

Another place where practitioners often take liberty is by applying modifications to learning algorithms through various heuristics that trade off between bias and variance. For instance, certain algorithms employ biased update rules to improve sample efficiency \citep{thomas2014bias}, or make partial corrections for off-policy sampling to mitigate variance \citep{munos2016safe,schulman2017proximal}. Regrettably, these heuristics could possibly result in suboptimal behavior for the agent \citep{nota2020policy}.

\yash{Trim intro down}

% Additionally, not only an improperly specified reward function but 
% % \dg{the comparision to a well-defined reward function here is misleading. Just go directly from rewards have to be correctly specified to the algorithm having to also correctly maximize reward function, but many algorithms introduce heuristics that can lead to incorrect optimization. }
% even a well-defined reward function one can lead to sub-optimal behavior in the agent due to the influence of its learning algorithm. Algorithms are often modified to  incorporate various heuristics and trade-offs between bias and variance. For instance, certain algorithms employ biased update rules to improve sample efficiency \citep{thomas2014bias}, or make partial corrections for off-policy sampling to mitigate variance \citep{schulman2017proximal}. Regrettably, these heuristics could possibly result in suboptimal behavior for the agent \citep{nota2020policy}.

%
% Additionally, let aside an ill-specified reward function, even a well-specified reward function can result in a sub-optimal behavior in the agent due to its learning algorithm.
% %
% Often algorithms employ various heuristics and bias-variance trade-offs.
% %
% For example, many algorithms use biased update rules to be more sample-efficient \citep{thomas2014bias}, or only partially correct for the off-policy sampling to mitigate variance \citep{schulman2017proximal}.
% % 
% Unfortunately, such heuristics can often lead to sub-optimal behavior in the agent \citep{nota2020policy}.
% Scotts points I want to incorporate
% \begin{itemize}
%     \item Our approach assumes that the agent is given a primary reward function that will induce desired behavior and given access to prior knowledge in the form of axuliary rewards. Instead of the human having to say how these auxiliary tasks are relevant it is part of the agent's part job to identify if any of these axualiary rewards are useful for maximizing the primary reward -- \textbf{Exlicitly stating out the assumption that agent is given a primary reward fdunciton which can induce desired behaiour. -- and agents part job to identify is a good way to explain it. }
% \end{itemize}

This raises the main question of our interest: \textit{Can we design a method that (i) allows for easy specification of auxiliary rewards by the users, (ii) when available, the agent should be able to make use of the auxiliary reward to maximize the primary reward, without leaving the onus on the designer to ensure optimality, and (iii) the algorithm being used to learn the policy maintain robutness to possible heuristic design choices made by the user.}
\yash{Talk about this much earlier}
% This raises the main question of our interest: \textit{Can we design a method that (i) allows for easy specification of auxiliary rewards by the users, (ii) leverages frequent evaluations when available to speed up learning but remain robust to its misspecification, and (iii) overcomes sub-optimality resulting due to agent's policy learning algorithm?}
%


To address this question, we draw inspiration from the optimal rewards framework of \citet{singh2009rewards,singh2010intrinsically}, and develop a bi-level optimization procedure.
%
This constitutes an inner-level process for optimizing a policy using a parameterized \textit{behavior alignment reward} $r_\phi$, and an outer-level process for optimizing $r_\phi$. 
%
Changing $r_\phi$ \textit{dynamically corrects} the inner policy optimization procedure to drive its learning towards a policy that exhibits the desired behavior, as illustrated in Figure \ref{fig:vectorfield}. 

%
This approach offers several advantages
%
\begin{figure}[t]
    \centering
    \includegraphics[width=0.25\textwidth]{images/1.png}
    \includegraphics[width=0.25\textwidth]{images/2.png}
    \includegraphics[width=0.25\textwidth]{images/3.png}
    \caption{
    Auxiliary rewards can be used to convey to the agent how we \textit{think} it should solve the problem. 
    %
    However, if not carefully designed, or if the algorithm uses sub-optimal heuristics, then it can result in policies with undesired behaviors.
    %
    This figure provides a visual illustration of a toy example of how the proposed method works.
    %
    %
    The star represents the optimal policy and the red dot represents the fix-point of a policy optimization process. 
    %
    \textbf{(Left)} Vector field of a policy optimization process that converges to a sub-optimal policy.
    %
    \textbf{(Middle and Right)} 
    % These vector fields show how 
    By changing the behavior alignment rewards, the proposed method can dynamically \textit{correct} the \textit{entire policy optimization process} to make it converge towards the policy with the desired behavior. \yash{Move this to later to explain the algorithm}}
    \label{fig:vectorfield}
\end{figure}
%

%
\textbf{A. Ease of reward specification:} Our method provides provision to separate the %separately specify a 
(sparse) \textit{primary reward function} that encodes the desired behavior, and freedom to \textit{optionally} specify a (dense) \textit{auxiliary reward function}
%
motivated by heuristics that can help in accelerating the agent's learning.
%
The primary rewards are used for the objective specified at the outer level, and the auxiliary rewards are only used for policy optimization in the inner level.
%
We show how policy optimization can benefit from this bi-level setup when auxiliary rewards are well-specified but remain robust against its ill-specification.
%


\textbf{B. Overcoming imperfections of the agent:}  
Our method can overcome imperfections of model-free policy optimization algorithms (e.g., using biased policy gradient updates, or improper off-policy correction) that may result in sub-optimal behavior.%
%

\textbf{C. Online optimization of behavior alignment rewards:} 
%
To enable efficient iterative bi-level optimization, the proposed method first develops regularizers specific for learning behavior alignment rewards $r_\phi$. 
%
% \dg{This is where we can start talking about using frodo or implicit gradient theorem}
Then it shows how the implicit gradient technique \citep{gould2016differentiating} can be used to update $r_\phi$ in the outer-level with respect to the fixed point of the policy optimization in the inner-level.
%\
%
\paragraph{Motivating Example: } 
% \yash{Not sure if we need this. Remove? Shrink?}
Consider the classic mountain-car problem \citep{sutton2018reinforcement}. 
% (for reference, see Figure \ref{fig:mc} in Section \ref{sec:experiments}).
%
It is easy to specify a reward function to only provide positive evaluation at the end of an episode, if the desired behavior is achieved (car reaches the flag).
%
However, a lack of evaluation at the intermediate steps provides minimal assistance to optimize the policy.
%
A common addition is to provide a small negative reward at every step to indicate that the agent should reach the flag quickly; however, this does not provide any information pertaining to \textit{how} to reach the flag quickly.
%

Herein lies the dilemma of designing a reward function that encodes the desired behavior but also provides frequent evaluations.
% to accelerate policy optimization.
%
A natural way to incorporate more evaluations might be to exploit the fact that the car would reach the flag quickly when it has a higher velocity.
%
Accordingly, one could provide positive evaluation proportional to the velocity magnitude attained by the car at any step.

Unfortunately, adding such rewards for the velocity can result in an optimal policy that keeps swinging the car between the hills to accumulate rewards from repeatedly attaining high-velocity, such that it surpasses the reward of reaching the flag itself.
%
To overcome such problems, we will show how it is possible to consider the two aspects of rewards \textit{separately}, instead of encoding them as a single reward function. 
%
That is, using a primary reward that encodes the desired behavior (reaching the flag) and an auxiliary reward that encodes information about ways that can accelerate policy optimization (attaining high velocity) \textit{even when it may not be perfectly aligned with the desired behavior}.
% \subsection{A Motivating Example} 
% % \yash{Not sure if we need this. Remove? Shrink?}
% Consider the classic mountain-car problem \citep{sutton2018reinforcement}. 
% % (for reference, see Figure \ref{fig:mc} in Section \ref{sec:experiments}).
% %
% It is easy to specify a reward function to only provide a positive reward at the end of an episode if the desired behavior is achieved (car reaches the flag in the fewest number of steps).
% %
% However, a lack of evaluation at the intermediate steps provides minimal assistance for the agent to learn a policy.
% %
% A common addition is to provide a small negative reward at every step to indicate that the agent should reach the flag quickly; however, this does not provide any information pertaining to \textit{how} to reach the flag quickly.
% %

% Herein lies the dilemma of designing a reward function that encodes the desired behavior but also provides frequent evaluations.
% % to accelerate policy optimization.
% %
% \dg{Either swap with Cartpole or change the example from Mountain Car.}
% A natural way to incorporate more evaluations might be to exploit the fact that the car would reach the flag quickly when it follows a \textit{energy pumping policy}. This policy chooses the action in agreement with the current velocity: left if
% velocity is negative, right otherwise.
% % pumping policy. A pumping policy  it has a higher velocity.
% %
% Accordingly, an auxiliary reward could provide positive feedback proportional to the agreement between the action taken by the agent w.r.t to heuristic energy pumping policy. 
% % Accordingly, one could provide positive evaluation proportional to the velocity magnitude attained by the car at any step.
% %

% %

% %
% Unfortunately, adding such rewards for the velocity can result in an optimal policy that keeps swinging the car between the hills to accumulate rewards from repeatedly attaining high-velocity, such that it surpasses the reward of reaching the flag itself.
% %
% To overcome such problems, we will show how it is possible to consider the two aspects of rewards \textit{separately}, instead of encoding them as a single reward function. 
% %
% That is, using a primary reward that encodes the desired behavior (reaching the flag) and an auxiliary reward that encodes information about ways that can accelerate policy optimization (attaining high velocity) \textit{even when it may not be perfectly aligned with the desired behavior}.
new intro outline
\begin{itemize}
    \item Problem description
    \item Motivating exmaple
    \item Why potential rewards not suffieicne
    \item Research questions
    \item COntributions
\end{itemize}

